Accelerating Construction of Non-Intrusive Nonlinear Structural Dynamics Reduced Order Models through Hyperreduction

We present a novel technique to significantly reduce the offline cost associated to non-intrusive nonlinear tensors identification in reduced order models (ROMs) of geometrically nonlinear, finite elements (FE)-discretized structural dynamics problems. The ROM is obtained by Galerkin-projection of the governing equations on a reduction basis (RB) of Vibration Modes (VMs) and Static Modal Derivatives (SMDs), resulting in reduced internal forces that are cubic polynomial in the reduced coordinates. The unknown coefficients of the nonlinear tensors associated with this polynomial representation are identified using a modified version of Enhanced Enforced Displacement (EED) method which leverages Energy Conserving Sampling and Weighting (ECSW) as hyperreduction technique for efficiency improvement. Specifically, ECSW is employed to accelerate the evaluations of the nonlinear reduced tangent stiffness matrix that are required within EED. Simulation-free training sets of forces for ECSW are obtained from displacements corresponding to quasi-random samples of a nonlinear second order static displacement manifold. The proposed approach is beneficial for the investigation of the dynamic response of structures subjected to acoustic loading, where multiple VMs must be added in the RB, resulting in expensive nonlinear tensor identification. Superiority of the novel method over standard EED is demonstrated on FE models of a shallow curved clamped panel and of a nine-bay aeronautical reinforced panel modelled, using the commercial finite element program Abaqus.

==> 5_Examples.tex <==
\section{Methodology Validation} \label{sec:examples}

\subsection{Flat Panel} %?

\subsection{Curved Panel}

\subsection{Nine Bay Panel}


==> introduction1.tex <==
\section{Introduction} \label{sec:Introduction}
The investigation of the response of aerospace panels subjected to acoustic loading has been of great interest for the aerospace community in the past decades \cite{Hollkamp2018}.
Experimental \cite{Hollkamp2018} and computational studies \cite{Gordon2011,Spottswood2008,Przekop2007,przekop2006nonlinear,mignolet2013review}  have been performed with the end goal of predicting fatigue life  and guarantee in service structural integrity.
With the advent of the \textit{Finite Element} (FE) method and the steady increase in computational power of modern computers, numerical investigations have become increasingly appealing compared to traditional experiments, which typically require costly testing facilities and instrumentation.\\
However, vibration assessment of real-life components using FEM is generally computationally demanding, if not intractable.  
This is due to the complex geometries that require large meshes, the necessity for simulations over extended time spans to obtain statistically relevant data, and the nonlinearities inherent in the \textit{equations of motion} (EOM).
In fact, the pursue of light-design structures leads to large in service structural displacements whose behavior can be accurately modelled only by assuming finite rotations in the FE formulation.
As a result, \textit{geometric nonlinearities} are introduced in the FE model within the \textit{Total Lagrangian} formulation, or with the adoption of \textit{von K\'arm\'an} strains in thin walled structures undergoing mild deformations. \\ \par
\textit{Reduced Order Models} (ROMs) have been successfully employed to speed up the dynamic analysis of thin walled structures. 
The core principal behind model reduction is the replacement of solutions of the starting FE model (referred to as \textit{High Fidelity Model} (HFM)) with accurate approximations computed in limited time using the ROM.
%GP
Among different approaches, \textit{Galerkin Projection} (GP) is arguably the most classical and established technique for model reduction, enjoying extensive application in academia as well as in an industrial setting. 
In GP ROMs, dimensionality reduction is achieved by restricting the HFM solution space to a small linear subspace spanned by few vectors constituting a \textit{reduction basis} (RB). \\\par
The choice of the RB dictates accuracy and efficiency of GP ROMs.
Different approaches, generally classifiable in  \textit{data-driven} and \textit{pyhsics-based} strategies, can be followed for RB construction.
%BASIS SELECTION
%data driven
Data-driven strategies rely on the availability of HFM solutions from which relevant vector components are usually extracted using \textit{Proper Orthogonal Decomposition} (POD) \cite{krysl2001dimensional} and stacked together to form the RB. 
This comes at the large cost of running HFM simulations. 
%Physics based approach
On the other hand, physics-based approaches are simulation free and harness information from the physics modelled in the equations to construct the RB.
Among these techniques, \textit{Modal Analysis}  \cite{geradin2015mechanical} represents the cornerstone for model reduction of linear structural systems and acts as the foundation for extending reduction to nonlinear systems.
As such, the RB for geometrically nonlinear structures can be constructed by complementing the RB of the underlying linearized system with additional vectors that capture the most prominent nonlinear effects. 
To this end, \textit{Modal Derivatives} vectors (MDs) \cite{Idelsohn1985,idelsohn1985load} have been successfully employed for model reduction of a large array of structures, both for transient and forced response \cite{Marconi2020,Marconi2021,Morteza,Sombroek2018,Wu2016,Rutzmoser2017,tiso2011reduction}.
\\ \par 
%Need for hyperreduction
Galerkin Projection usually enables a dramatic reduction in the number of degrees of freedom of the model, from hundreds of thousands, if not millions, to usually far less than a hundred. 
However, for nonlinear systems, the speed up in time integration of the ROM with respect to the HFM is generally small \cite{Farhat2014,Rutzmoser2017,Jain2018,An2008,rutzmoserThesis}, since another computational bottleneck arises:
the construction of the reduced internal force vector and of its Jacobian.
%In fact, these operations still retain the high dimensionality of the HFM, since the reduced forces and the reduced tangent stiffness matrix are computed by projecting the internal forces and tangent stiffness matrix of the HFM onto the RB. \par
For FE structures with geometric nonlinearities, with linear elastic material, a solution to this problem is easily obtained by exploiting the polynomial nature of the internal forces \cite{Mignolet2008, mignolet2013review}. 
In an exact formulation, the reduced forces are expressed as third order polynomials in the reduced coordinates. The generally expensive computation of the associated tensors is performed once and for all during model construction, and the reduced order forces and Jacobians are computed \textit{on the fly} during time integration through tensor contractions.\\ \par
The reduced order tensors can be obtained following different approaches that fall in two different categories: \textit{direct methods} and \textit{indirect methods} \cite{mignolet2013review}.
The direct methods, were the first to be employed \cite{nashThesis, shi1996finite, almroth1978automatic} and consist in contracting the HFM nonlinear stiffness operators onto the reduction basis, relying on the availability of the decomposition of the internal forces into their linear, quadratic and cubic components.
This separation is not generally available in commercial FE packages like ABAQUS, NASTRAN or ANSYS, and as such, has limited the use of tensorial formulation to ROM constructed from \textit{ad-hoc} written FE codes. 
This limitation was overcome in \cite{Muravyov2003,McEwan2001,Hollkamp2008} with the development \textit{indirect} methods for identification of the reduced order tensors. 
As opposed to the direct methods, in an indirect scheme the FE code is used as a black-box exchanging forces to displacements inputs and displacements to forces inputs. 
More specifically, the reduced tensors are identified in \cite{McEwan2001,Hollkamp2008} by running a set of nonlinear static analysis to prescribed loads and reading the displacements (\textit{Implicit Condensation} (IC)), or in \cite{Muravyov2003} by reading the internal force resulting from some imposed displacements (\textit{Enforced Displacement Method} (ED)).\\ \par
Albeit these methods are well established, their applicability to large ROMs, featuring many vectors in the reduction basis, is hindered by the high computational cost for identifying the tensors coefficients \cite{Perez2014}. 
As such, constructing a ROM for an aerospace component subjected to acoustic loading can be extremely problematic, since the high modal density and the large excitation bandwidth of the load, force the analyst to include a large number of vectors in the basis to effectively capture  the complex dynamics \cite{Perez2014}.
In this regard, the \textit{Enhanced Enforced Displacement} (EED) method was  was proposed in \cite{Perez2014}. In the EED scheme, the number of total nonlinear static analysis required by the ED method for tensor identifications, was significantly reduced by exploiting the availability of the tangent stiffness matrix, allowing in this way for faster tensor construction.
\\ \par
%why we still need to accelerate tensor construction
Even with EED, model construction time for multi-modes ROMs can still be large and remains the bottleneck cost in the construction of \textit{physics-based} ROMs. 
Moreover, in the context of geometry optimization or of quantification of uncertainties in presence of structural defects \cite{Wang2018,Perez2011}, a different ROM may be required for each tested geometry configuration. 
Therefore, these applications would certainly benefit from a reduction of total model construction time.\\ \par
To this end, one could consider abandoning the tensorial formulation and resorting to \textit{hyperreduction} techniques \cite{farhat2020}, where the reduced order forces and their Jacobians are replaced with a quickly computable approximated version. 
Within these methods, \textit{Discrete Empirical Interpolation} (DEIM) \cite{chaturantabut2010nonlinear} and \textit{Energy Conserving Sampling and Weighting} (ECSW) \cite{Farhat2014,Farhat2015} have enjoyed successful  application in the field of model reduction for structural vibrations. 
While both the approaches have been designed to rely on training data coming from expensive HFM simulations, alternative, less computationally expensive training strategies have been proposed in  \cite{Rutzmoser2017, Jain2018} for ECSW only.
Specifically, ECSW was trained in \cite{Rutzmoser2017,rutzmoserThesis} with nonlinear static solutions, whereas in \cite{Jain2018} with displacements obtained from a linear run lifted on a second order nonlinear manifold.\\ \par
Physics-based ROM, equipped with ECSW hyperreduction, constructed with simulations-free training, allow potentially for a significant reduction in model construction time when compared to ROM in the tensorial formulation, as reported in  \cite{rutzmoserThesis}. 
The drawback of ECSW-ROMs lies, however, in the \textit{semi-intrusive} nature of ECSW: during solution of the ROMs equations, long time is spent for communication between the ROM time integrator solver and the commercial FE software, thus severely undermining the online performance of the ECSW-ROM, as reported in \cite{Trainotti2024}.
Conversely, a ROM in the tensorial formulation, once constructed, does not retain any bound with the underlying FE code, and time integration of the ROM can be implemented in a \textit{stand-alone} code. 
For the above mentioned reasons, ECSW-ROMs can be efficient only if the ROM solver is integrated in the FE package as in  \cite{Farhat2015}, leaving out the possibility of their use with commercial FE packages.  
%what we propose
\\ \par
As such, towards the goal of fully non-intrusive ROMs, we propose a new method to accelerate ROM tensor identification from commercial FE packages. Our approach is based on EED identification procedure and ECSW trained with the second order manifold as in \cite{Jain2018}. The idea is to cheaply construct a hyperreduced mesh to use for a fast evaluation of the tangent stiffness in the EED scheme.
Our method shares some similarities with the recent work proposed in \cite{Kim2023}. In that work, ECSW was trained using a comparable hyperreduction strategy based on the same manifold we use \cite{Jain2018} and was employed to accelerate tensor construction for a parametric ROM.
However, the greatest distinctive feature of the method here proposed from the one presented in \cite{Kim2023}, is its non-intrusiveness, that allows for the use of commercial FE packages, making it relevant in an industrial setting. \\ \par
%content
In the following, we first recall the preliminaries in section 1, focusing on ROMs based on MDs, tensor idenfication based on EED and ECSW hyperreduction strategy. In section 2 we illustrate the core of the proposed approach for tensor identification. Eventually, in section 3, we provide the application of the methodology to two case study: a rectangular curved panel and an aerospace multi-bay stiffened panel subjected to acoustic loading.
